Compressing Context to Enhance Inference Efficiency of Large Language Models

Large language models (LLMs) achieved remarkable performance across various tasks. However, they face challenges in managing long documents and extended conversations, due to significantly increased computational requirements, both in memory and inference time, and potential context truncation when the input exceeds the LLM's fixed context length. This paper proposes a method called Selective Context that enhances the inference efficiency of LLMs by identifying and pruning redundancy in the input context to make the input more compact. We test our approach using common data sources requiring long context processing: arXiv papers, news articles, and long conversations, on tasks of summarisation, question answering, and response generation. Experimental results show that Selective Context significantly reduces memory cost and decreases generation latency while maintaining comparable performance compared to that achieved when full context is used. Specifically, we achieve a 50\% reduction in context cost, resulting in a 36\% reduction in inference memory usage and a 32\% reduction in inference time, while observing only a minor drop of .023 in BERTscore and .038 in faithfulness on four downstream applications, indicating that our method strikes a good balance between efficiency and performance.

==> tex_file/text_2.tex <==
\colorize{16.590300204199682}{\sdelete{INTRODUCTION}}
\colorize{41.72455108787692}{ In}
\colorize{25.125269672703226}{\sdelete{ the past many years}}
\colorize{5.017680070948296}{\sdelete{,}}
\colorize{39.19774073953673}{ researchers}
\colorize{2.297892749966565}{\sdelete{ have}}
\colorize{23.37555448005995}{\sdelete{ focused}}
\colorize{2.370216775265276}{\sdelete{ on}}
\colorize{28.31743449807127}{ how}
\colorize{10.475525440663304}{\sdelete{ to}}
\colorize{58.329768321217244}{ turn}
\colorize{72.22844856507236}{ vehicles}
\colorize{21.72660338800466}{\sdelete{ from}}
\colorize{46.12210294766961}{ assisted driving}
\colorize{5.833565169541879}{\sdelete{ to}}
\colorize{28.80451339552923}{ more intelligent autonomous driving}
\colorize{4.884433406993603}{\sdelete{.}}
\colorize{73.98864557429393}{Due}
\colorize{0.5399346119660673}{\sdelete{ to}}
\colorize{55.21327617409655}{ the iteration}
\colorize{5.241610484686979}{\sdelete{ of}}
\colorize{61.14101939555946}{ intelligent hardware}
\colorize{10.941169927327433}{\sdelete{ and}}
\colorize{28.25537322917023}{ the improvement}
\colorize{2.059014806850694}{\sdelete{ of}}
\colorize{35.927574362353724}{ chip computing power}
\colorize{1.6451788636777172}{\sdelete{,}}
\colorize{20.820076121716806}{\sdelete{ a large amount}}
\colorize{0.03910628706618764}{\sdelete{ of}}
\colorize{13.710874234103681}{\sdelete{ data}}
\colorize{46.51484477942384}{ collected}
\colorize{12.133073768039123}{\sdelete{ by}}
\colorize{18.377120808809323}{\sdelete{ sensors}}
\colorize{16.518775486472386}{\sdelete{ can}}
\colorize{1.622035263070444}{\sdelete{ be}}
\colorize{37.5327046191736}{ quickly}
\colorize{37.34382564443663}{ converted}
\colorize{18.395091361136924}{\sdelete{ and}}
\colorize{44.124147393232235}{ fed}
\colorize{4.091927750351686}{\sdelete{ into}}
\colorize{42.78537028189594}{ models}
\colorize{13.328704912633093}{\sdelete{ to}}
\colorize{18.170150608207486}{\sdelete{ make}}
\colorize{13.8434612663353}{\sdelete{ decisions}}
\colorize{5.838042459458259}{\sdelete{.}}
\colorize{33.097980030436005}{In}
\colorize{45.26408443213671}{ the driving process}
\colorize{6.754881229224781}{\sdelete{,}}
\colorize{32.739679683233256}{ the safety factor}
\colorize{6.519467069154183}{\sdelete{ is}}
\colorize{20.724957971402798}{\sdelete{ the first consideration}}
\colorize{20.72091691632363}{\sdelete{ for}}
\colorize{46.0660523522388}{ users}
\colorize{19.420335996370188}{\sdelete{ and}}
\colorize{43.65108450086473}{ researchers}
\colorize{4.291175221673357}{\sdelete{.}}
\colorize{79.16530651798905}{Therefore}
\colorize{2.946039746237614}{\sdelete{,}}
\colorize{47.230947946891334}{ how}
\colorize{93.34991516629778}{ AV}
\colorize{40.380511856106274}{ should}
\colorize{57.5045197103415}{ avoid}
\colorize{58.006140749512404}{ collisions}
\colorize{38.57093976069346}{ has}
\colorize{10.326034308489668}{\sdelete{ become}}
\colorize{17.163959570298772}{\sdelete{ a top priority}}
\colorize{10.540729123895687}{\sdelete{.}}
\colorize{30.44850754549784}{Concepts}
\colorize{34.36135880726982}{ such}
\colorize{0.0}{\sdelete{ as}}
\colorize{26.519821444343183}{ probabilistic methods}
\colorize{28.699753907253832}{ (}
\colorize{48.262297154691005}{eg}
\colorize{33.186211241417}{.}
\colorize{33.186211241417}{:}
\colorize{11.932224844238084}{\sdelete{ Markov chains}}
\colorize{22.48926994824511}{\sdelete{ and}}
\colorize{11.877831927612897}{\sdelete{ Monte Carlo}}
\colorize{30.97773466754375}{ )}
\colorize{30.97773466754375}{,}
\colorize{42.42376146854651}{ safety distance-based control methods}
\colorize{31.5489436103978}{ ,}
\colorize{9.801123276626601}{\sdelete{ and}}
\colorize{32.35719283951772}{ trajectory prediction methods}
\colorize{16.593774089882658}{\sdelete{ have}}
\colorize{4.1511075614457145}{\sdelete{ been}}
\colorize{47.12151665804168}{ designed}
\colorize{19.673441198687698}{\sdelete{ in}}
\colorize{8.547311724090038}{\sdelete{ recent years}}
\colorize{6.115169690313368}{\sdelete{ to}}
\colorize{25.759290511570583}{ cope}
\colorize{0.14393201530881977}{\sdelete{ with}}
\colorize{35.70870524817114}{ complex traffic conditions}
\colorize{6.0167699237147225}{\sdelete{.}}
\colorize{33.097980030436005}{In}
\colorize{47.16323500829344}{ terms}
\colorize{0.000989465685643769}{\sdelete{ of}}
\colorize{65.50528836246002}{ vision}
\colorize{3.991609877878212}{\sdelete{,}}
\colorize{73.56374273643932}{ CNN}
\colorize{14.26898783553564}{\sdelete{ has}}
\colorize{34.825371184342444}{ made}
\colorize{47.74596186317465}{ outstanding contributions}
\colorize{35.95158487662464}{ and}
\colorize{16.778357086692992}{\sdelete{ has}}
\colorize{13.653248094801942}{\sdelete{ been}}
\colorize{86.21463974973292}{ applied}
\colorize{8.898415076389979}{\sdelete{ to}}
\colorize{12.880084696641845}{\sdelete{ a large number}}
\colorize{0.057342590428600765}{\sdelete{ of}}
\colorize{51.78776643813816}{ road condition inspection tasks}
\colorize{46.19542343470229}{ due}
\colorize{0.07917659655689631}{\sdelete{ to}}
\colorize{34.54930251181235}{ its excellent regional feature extraction capabilities}
\colorize{3.7712245509805333}{\sdelete{.}}
\colorize{56.577958122835604}{The local feature information}
\colorize{63.78537745944482}{ obtained}
\colorize{12.074816355295564}{\sdelete{ by}}
\colorize{59.099688115256946}{ CNN}
\colorize{33.825397850441306}{ will}
\colorize{5.536622287974388}{\sdelete{ be}}
\colorize{10.611970255039365}{\sdelete{ used}}
\colorize{18.315879742856882}{\sdelete{ for}}
\colorize{55.977694386151356}{ obstacle detection}
\colorize{16.998969430682646}{\sdelete{.}}
\colorize{83.90671309696106}{Secondly}
\colorize{1.5045229199559071}{\sdelete{,}}
\colorize{40.41945999446819}{ because}
\colorize{53.80904146229321}{ the motion trajectory}
\colorize{11.865544306970396}{\sdelete{ is}}
\colorize{57.69757474367745}{ planned}
\colorize{26.180295594171515}{ for}
\colorize{90.16305526275936}{ AV}
\colorize{20.999703709999977}{\sdelete{,}}
\colorize{32.86634792986521}{ the relationship}
\colorize{1.7409314299735685}{\sdelete{ between}}
\colorize{49.49529058624467}{ each local feature}
\colorize{15.010071179426616}{\sdelete{ of}}
\colorize{12.600737952612265}{\sdelete{ the image}}
\colorize{51.84262293120726}{ obtained}
\colorize{7.251573508608009}{\sdelete{ by}}
\colorize{69.6689628396792}{ CNN}
\colorize{53.41350276990966}{ needs}
\colorize{0.2812656807919917}{\sdelete{ to}}
\colorize{0.4242728578822596}{\sdelete{ be}}
\colorize{38.46220536152151}{ established}
\colorize{6.8629811118536}{\sdelete{.}}
\colorize{60.04703571955675}{Some strategies}
\colorize{15.301060330349292}{\sdelete{ are}}
\colorize{32.63812334830295}{ based}
\colorize{0.998776957597443}{\sdelete{ on}}
\colorize{100.0}{ CNN}
\colorize{85.9136874898898}{ plus}
\colorize{28.3640804767963}{ RNN}
\colorize{51.48748372787445}{ so}
\colorize{9.921630887777978}{\sdelete{ that}}
\colorize{12.882565794848656}{\sdelete{ they}}
\colorize{9.79983357819708}{\sdelete{ can}}
\colorize{31.43424115059848}{ deal}
\colorize{0.6745919495713892}{\sdelete{ with}}
\colorize{48.28943587901232}{ sequential graphs}
\colorize{30.073265387872667}{ as}
\colorize{27.498675106661956}{ input}
\colorize{16.874780522435074}{\sdelete{,}}
\colorize{47.98450139243944}{ eg}
\colorize{20.35547294711799}{\sdelete{.}}
\colorize{20.35547294711799}{\sdelete{:}}
\colorize{71.9904954337777}{ STDN}
\colorize{33.782435808546104}{ .}
\colorize{53.44210541507992}{Although}
\colorize{44.897495572746266}{ the above strategies}
\colorize{19.083168853784198}{\sdelete{ have}}
\colorize{45.97716497889891}{ performed}
\colorize{4.546362872139257}{\sdelete{ well}}
\colorize{8.294556399609641}{\sdelete{ in}}
\colorize{23.11761177731732}{\sdelete{ a large number}}
\colorize{0.01383274723993188}{\sdelete{ of}}
\colorize{56.440578088545735}{ vision tasks}
\colorize{1.7352518545212252}{\sdelete{,}}
\colorize{32.81402652384068}{ their performances}
\colorize{11.682053405672312}{\sdelete{ are}}
\colorize{14.218624734758043}{\sdelete{ still}}
\colorize{13.724693616749361}{\sdelete{ far}}
\colorize{38.346034455615595}{ inferior}
\colorize{1.0031671363041088}{\sdelete{ to}}
\colorize{25.03094482519514}{\sdelete{ similar-sized convolutional neural networks counterparts}}
\colorize{19.34412688653923}{\sdelete{,}}
\colorize{16.81690624817233}{\sdelete{ such}}
\colorize{0.040663011144759245}{\sdelete{ as}}
\colorize{34.07229452559663}{ EfficientNets}
\colorize{16.51933133895341}{\sdelete{ and}}
\colorize{52.48500990300112}{ RepVGG}
\colorize{37.00120330375665}{ .}
\colorize{36.84382992697078}{We}
\colorize{39.11587128659842}{ believe}
\colorize{32.976306411230794}{ this}
\colorize{8.948033772284573}{\sdelete{ is}}
\colorize{42.03215095120414}{ due}
\colorize{0.35246895061335315}{\sdelete{ to}}
\colorize{29.216495843450463}{ the following aspects}
\colorize{23.604122981203414}{\sdelete{.}}
\colorize{52.242311787659915}{First}
\colorize{15.846641984936264}{\sdelete{,}}
\colorize{44.20623380713441}{ the huge differences}
\colorize{6.084919097149825}{\sdelete{ between}}
\colorize{52.38056871632059}{ the sequential tasks}
\colorize{18.085211522165}{\sdelete{ of}}
\colorize{39.806578708148464}{ NLP}
\colorize{5.651160330079183}{\sdelete{ and}}
\colorize{32.50351050906449}{ the image tasks}
\colorize{3.351719289605881}{\sdelete{ of}}
\colorize{50.2957465674861}{ CV}
\colorize{15.14623769045736}{\sdelete{ are}}
\colorize{45.160355973535644}{ ignored}
\colorize{4.714102407460046}{\sdelete{.}}
\colorize{41.03777385259368}{For}
\colorize{40.03911435182953}{ example}
\colorize{2.1831833514388537}{\sdelete{,}}
\colorize{26.934458441082814}{ when}
\colorize{48.15213824212212}{ the local feature information}
\colorize{63.483388161390806}{ acquired}
\colorize{16.41740518991204}{\sdelete{ in}}
\colorize{17.306830612554812}{\sdelete{ a two-dimensional image}}
\colorize{5.638424746640065}{\sdelete{ is}}
\colorize{35.455455237608916}{ compressed}
\colorize{13.271887286031028}{\sdelete{ into}}
\colorize{16.916088658081097}{\sdelete{ one-dimensional time series information}}
\colorize{4.510957557989514}{\sdelete{,}}
\colorize{44.10696649836411}{ how}
\colorize{11.228309592411348}{\sdelete{ to}}
\colorize{35.44812205759124}{ achieve}
\colorize{47.13785095262492}{ accurate mapping}
\colorize{42.22326766584777}{ becomes}
\colorize{12.432802171951499}{\sdelete{ a difficult problem}}
\colorize{1.2648929544399923}{\sdelete{.}}
\colorize{61.914096688122655}{Second}
\colorize{24.08365623779715}{\sdelete{,}}
\colorize{22.55950798061027}{\sdelete{ it}}
\colorize{10.921670592124604}{\sdelete{ is}}
\colorize{34.90191893428735}{ difficult}
\colorize{1.2614958435240575}{\sdelete{ to}}
\colorize{38.159163941064485}{ keep}
\colorize{35.731930630240235}{ the original information}
\colorize{28.611673538194417}{ of}
\colorize{71.34652864425848}{ inputs}
\colorize{50.00738206599894}{ since}
\colorize{63.059982429607906}{ after}
\colorize{45.860120698267046}{ RNN layers}
\colorize{7.705284890855831}{\sdelete{,}}
\colorize{18.59035019494718}{\sdelete{ we}}
\colorize{16.775396813981953}{\sdelete{ need}}
\colorize{1.0801600961805684}{\sdelete{ to}}
\colorize{58.093195393505056}{ recover}
\colorize{36.18923602239229}{ the dimension}
\colorize{38.51188514839434}{ from}
\colorize{39.57303317780242}{ one}
\colorize{20.77522830439862}{\sdelete{ to}}
\colorize{43.496373483994766}{ three}
\colorize{8.135341997170869}{\sdelete{.}}
\colorize{71.33078074764538}{Besides}
\colorize{20.62722447357178}{\sdelete{,}}
\colorize{58.91281760070582}{ due}
\colorize{0.15375668905573978}{\sdelete{ to}}
\colorize{42.364910593402804}{ the several transformations}
\colorize{40.989988640255916}{ between}
\colorize{34.23342751094781}{ different dimensions}
\colorize{3.578910076058586}{\sdelete{,}}
\colorize{43.27996246462596}{ that process}
\colorize{35.918636475693624}{ becomes}
\colorize{21.539609937287455}{\sdelete{ even}}
\colorize{17.27005725268148}{\sdelete{ harder}}
\colorize{18.42101203694147}{\sdelete{,}}
\colorize{29.348512190412094}{ especially}
\colorize{16.02401322947579}{\sdelete{ since}}
\colorize{52.391649815283145}{ our input size}
\colorize{6.227746033227997}{\sdelete{ is}}
\colorize{33.47063394180939}{ 224×224×5}
\colorize{8.773006611206421}{\sdelete{.}}
\colorize{67.10294565908157}{Third}
\colorize{27.784454931822815}{,}
\colorize{39.43609631707816}{ the computational and memory requirement}
\colorize{9.548510573183055}{\sdelete{ of}}
\colorize{62.90236016365143}{ switching}
\colorize{8.805504749001527}{\sdelete{ between}}
\colorize{56.1470072781352}{ layers}
\colorize{34.46059997010705}{ are}
\colorize{38.512556646348585}{ extremely heavy tasks}
\colorize{14.020255540524776}{\sdelete{,}}
\colorize{11.095471408380298}{\sdelete{ which}}
\colorize{39.69999154373023}{ also}
\colorize{46.30445800929819}{ becomes}
\colorize{37.475396253519996}{ a tricky point}
\colorize{9.611772920884686}{\sdelete{ for}}
\colorize{25.04688146276262}{\sdelete{ the algorithm}}
\colorize{9.253178683338053}{\sdelete{ to}}
\colorize{23.624265657201786}{\sdelete{ run}}
\colorize{10.03294468380897}{\sdelete{.}}
\colorize{56.463772548020906}{Higher hardware requirements}
\colorize{50.192045763237324}{ as}
\colorize{7.249270604991224}{\sdelete{ well}}
\colorize{0.30104226344668555}{\sdelete{ as}}
\colorize{20.92620749212866}{\sdelete{ more}}
\colorize{65.05540987343959}{ running}
\colorize{15.508503420375286}{\sdelete{ time}}
\colorize{84.16996241850491}{ arise}
\colorize{12.026306347524596}{\sdelete{ when}}
\colorize{22.94347986304376}{\sdelete{ running}}
\colorize{56.072032558029186}{ the attention part}
\colorize{21.075414287280115}{\sdelete{.}}
\colorize{33.097980030436005}{In}
\colorize{22.86998779332528}{\sdelete{ this paper}}
\colorize{3.936507776450292}{\sdelete{,}}
\colorize{3.833868145119837}{\sdelete{ we}}
\colorize{19.218324723940345}{\sdelete{ propose}}
\colorize{22.98727247826967}{\sdelete{ a new network structure}}
\colorize{24.441673504993737}{\sdelete{ based}}
\colorize{0.25918053794845525}{\sdelete{ on}}
\colorize{64.05191136383111}{ CNN}
\colorize{22.89873562384507}{\sdelete{ and}}
\colorize{45.209390156984114}{ attention}
\colorize{26.204378261161594}{ to}
\colorize{56.85700587303628}{ vision tasks}
\colorize{24.349352215309054}{\sdelete{ in}}
\colorize{22.38294532419138}{\sdelete{ autonomous driving}}
\colorize{3.306519507804015}{\sdelete{.}}
\colorize{41.705951147631524}{The new network structure}
\colorize{43.68104246070041}{ overcomes}
\colorize{18.073955697976597}{\sdelete{ these problems}}
\colorize{9.83006607033003}{\sdelete{ by}}
\colorize{19.69596943967588}{\sdelete{ using}}
\colorize{28.903937255085044}{ Sequential Spatial Network (SSN) blocks}
\colorize{14.560438562738351}{\sdelete{.}}
\colorize{39.48892221390942}{As}
\colorize{53.75507977607309}{ shown}
\colorize{3.0704541631579514}{\sdelete{ in}}
\colorize{27.249888508559327}{ Fig}
\colorize{0.9178230397021774}{\sdelete{.}}
\colorize{60.963800124255926}{,}
\colorize{81.3493844110465}{ input images}
\colorize{65.79245367067062}{ first}
\colorize{35.13526837013534}{ go}
\colorize{3.2843600753141002}{\sdelete{ through}}
\colorize{39.94872879012716}{ the convolution stem}
\colorize{36.74581586316562}{ for}
\colorize{16.374649165399298}{\sdelete{ fine-grained feature extraction}}
\colorize{9.578889381979943}{\sdelete{,}}
\colorize{10.820001628559526}{\sdelete{ and}}
\colorize{25.490002987905825}{\sdelete{ are}}
\colorize{1.7088498421449116}{\sdelete{ then}}
\colorize{20.631953367813356}{\sdelete{ fed}}
\colorize{7.679339326134222}{\sdelete{ into}}
\colorize{29.969554401794184}{ a stack}
\colorize{1.9577038665864896}{\sdelete{ of}}
\colorize{59.53415055989176}{ SSN}
\colorize{36.44869574234026}{ blocks}
\colorize{12.901963311754413}{\sdelete{ for}}
\colorize{19.652013349517453}{\sdelete{ further processing}}
\colorize{2.5573825628778866}{\sdelete{.}}
\colorize{33.34371201390263}{The Upsampling Convolutional Decreasing (UCD) blocks}
\colorize{9.065329204715875}{\sdelete{ are}}
\colorize{38.96012700256563}{ introduced}
\colorize{26.452771161848897}{ for}
\colorize{13.679611868751133}{\sdelete{ the purpose}}
\colorize{0.1903693494879159}{\sdelete{ of}}
\colorize{46.0748766046513}{ local information enhancement}
\colorize{24.987602096000344}{\sdelete{ by}}
\colorize{25.96773729368665}{ deep convolution}
\colorize{50.68685327281038}{,}
\colorize{16.756723338299786}{\sdelete{ and}}
\colorize{36.004402175466375}{ in}
\colorize{59.58317343019611}{ SSN block}
\colorize{31.59847557218748}{ of}
\colorize{65.99482319266421}{ features}
\colorize{51.143119163000186}{ generated}
\colorize{28.38733766137052}{ in}
\colorize{12.731049986982592}{\sdelete{ the first stage}}
\colorize{47.273832305196926}{ can}
\colorize{2.3020200112039144}{\sdelete{ be}}
\colorize{55.48187284176045}{ less loss}
\colorize{26.40162443728869}{ of}
\colorize{33.6034169931181}{ image resolution}
\colorize{16.63805222754366}{\sdelete{,}}
\colorize{20.34397426743584}{\sdelete{ which}}
\colorize{8.781235038028687}{\sdelete{ is}}
\colorize{50.77630932019462}{ crucial}
\colorize{3.812301219697894}{\sdelete{ for}}
\colorize{45.176400877892334}{ the subsequent trajectory adjustment task}
\colorize{2.6932469375397026}{\sdelete{.}}
\colorize{33.097980030436005}{In}
\colorize{33.20125847730435}{ addition}
\colorize{19.239640950088617}{\sdelete{,}}
\colorize{25.81696341186801}{ we}
\colorize{69.87646852910265}{ adopt}
\colorize{43.06673477545972}{ a staged architecture design}
\colorize{41.050290715246504}{ using}
\colorize{28.756435528745723}{ five convolutional layers}
\colorize{19.778249936850493}{\sdelete{ with}}
\colorize{21.11499118505183}{\sdelete{ different kernel sizes}}
\colorize{11.048990978664206}{\sdelete{ and}}
\colorize{57.36482198992654}{ steps}
\colorize{82.23279766688404}{ gradually}
\colorize{25.013716603674123}{\sdelete{ decreasing}}
\colorize{23.907733075704808}{\sdelete{ the resolution}}
\colorize{28.734446040798346}{ (}
\colorize{33.37834085956405}{sequence length}
\colorize{4.497358404549343}{\sdelete{)}}
\colorize{23.276433990759987}{\sdelete{ and}}
\colorize{51.744110349935454}{ flexibly}
\colorize{15.676923705288171}{\sdelete{ increasing}}
\colorize{15.02975258082879}{\sdelete{ the dimensionality}}
\colorize{12.88022171138728}{\sdelete{.}}
\colorize{46.16600398052667}{Such a design}
\colorize{47.72563402871753}{ helps}
\colorize{11.963709966906745}{\sdelete{ to}}
\colorize{58.33438710085607}{ extract}
\colorize{52.64898424797699}{ local features}
\colorize{11.466970926527829}{\sdelete{ of}}
\colorize{41.02032596752436}{ different scales}
\colorize{13.27336478265292}{\sdelete{ and}}
\colorize{39.249462171818166}{,}
\colorize{42.83143212527965}{ since}
\colorize{27.634622142696795}{ the first stage}
\colorize{64.12726444575709}{ retains}
\colorize{27.590154321319403}{ high resolution}
\colorize{9.179160552418061}{\sdelete{,}}
\colorize{44.83387748951291}{ our design}
\colorize{10.075790577424561}{\sdelete{ can}}
\colorize{36.52144604690936}{ effectively}
\colorize{27.6034023901871}{ reduce}
\colorize{16.541217860696705}{\sdelete{ the resolution}}
\colorize{5.548146610783205}{\sdelete{ of}}
\colorize{26.903851458739215}{ the output information}
\colorize{23.785897301433902}{\sdelete{ in}}
\colorize{24.54747604001655}{\sdelete{ the first layer}}
\colorize{43.66255301216256}{ at}
\colorize{17.05415961142373}{\sdelete{ each convolutional layer}}
\colorize{16.51697594234792}{\sdelete{,}}
\colorize{23.305646791503047}{\sdelete{ thus}}
\colorize{15.890948028352762}{\sdelete{ reducing}}
\colorize{14.721828306808893}{\sdelete{ the computational effort}}
\colorize{14.486707785678973}{\sdelete{ of}}
\colorize{17.32767848962077}{\sdelete{ subsequent layers}}
\colorize{2.6977999501007153}{\sdelete{.}}
\colorize{54.342557774379294}{The Reinforcement Region Unit}
\colorize{8.239640889638716}{\sdelete{ (}}
\colorize{0.2940172723300369}{\sdelete{RRU}}
\colorize{0.5468819836009182}{\sdelete{)}}
\colorize{35.61972963230714}{ and}
\colorize{30.21438659721652}{ the Fast MultiHead Self-Attention (FMHSA}
\colorize{0.17623253510246026}{\sdelete{)}}
\colorize{43.03959397706198}{ in}
\colorize{39.64704263531193}{ the SSN block}
\colorize{34.96603655568434}{ can}
\colorize{39.953217419584995}{ help}
\colorize{54.21605268842584}{ obtain}
\colorize{25.458733035204617}{\sdelete{ global and local structural information}}
\colorize{42.62179353108504}{ within}
\colorize{49.74201819211772}{ the intermediate features}
\colorize{27.370659338863863}{ and}
\colorize{32.27266354069554}{ improve}
\colorize{30.17914319929943}{ the normalization capability}
\colorize{6.158196895918697}{\sdelete{ of}}
\colorize{19.479843700091262}{\sdelete{ the network}}
\colorize{3.149932997902072}{\sdelete{.}}
\colorize{62.424960566038465}{Finally}
\colorize{5.6999865779387475}{\sdelete{,}}
\colorize{62.67687663120751}{ average pooling}
\colorize{19.32402342944047}{\sdelete{ is}}
\colorize{22.82931817153331}{\sdelete{ used}}
\colorize{6.215327972033808}{\sdelete{ to}}
\colorize{25.214389154049936}{\sdelete{ obtain}}
\colorize{65.1216546173341}{ better trajectory tuning}
\colorize{10.212147149276497}{\sdelete{.}}
\colorize{46.831458955984765}{Extensive experiments}
\colorize{18.013116625745173}{\sdelete{ on}}
\colorize{72.7198287576347}{ the lykit dataset}
\colorize{28.168677211846134}{ demonstrate}
\colorize{18.496299879736373}{\sdelete{ the superiority}}
\colorize{0.16121209628247685}{\sdelete{ of}}
\colorize{45.172928459147045}{ our SSN network}
\colorize{23.449412718543062}{\sdelete{ in}}
\colorize{16.062328585976683}{\sdelete{ terms}}
\colorize{0.03506349277966617}{\sdelete{ of}}
\colorize{10.317795322732891}{\sdelete{ accuracy}}
\colorize{20.051687875987565}{\sdelete{.}}
\colorize{33.097980030436005}{In}
\colorize{33.20125847730435}{ addition}
\colorize{0.6957146455342755}{\sdelete{ to}}
\colorize{61.445992723927155}{ image classification}
\colorize{3.320561231442106}{\sdelete{,}}
\colorize{58.465259563245716}{ SSN block}
\colorize{29.33936890733544}{ can}
\colorize{7.045547201330467}{\sdelete{ be}}
\colorize{39.32449697728961}{ easily}
\colorize{49.29742419841668}{ transferred}
\colorize{2.9256548181131823}{\sdelete{ to}}
\colorize{17.028600817758097}{\sdelete{ other vision tasks}}
\colorize{30.355012454260056}{ and}
\colorize{41.772107020493884}{ serve}
\colorize{1.162913407358378}{\sdelete{ as}}
\colorize{28.053110176432945}{ a versatile backbone}
\colorize{25.491883232458328}{.}
